MUFFIN: Curating Multi-Faceted Instructions for Improving Instruction-Following

In the realm of large language models (LLMs), enhancing instruction-following capability often involves curating expansive training data. This is achieved through two primary schemes: i) Scaling-Inputs: Amplifying (input, output) pairs per task instruction, aiming for better instruction adherence. ii) Scaling Input-Free Tasks: Enlarging tasks, each composed of an (instruction, output) pair (without requiring a separate input anymore). However, LLMs under Scaling-Inputs tend to be overly sensitive to inputs, leading to misinterpretation or non-compliance with instructions. Conversely, Scaling Input-Free Tasks demands a substantial number of tasks but is less effective in instruction following when dealing with instances in Scaling-Inputs. This work introduces MUFFIN, a new scheme of instruction-following dataset curation. Specifically, we automatically Scale Tasks per Input by diversifying these tasks with various input facets. Experimental results across four zero-shot benchmarks, spanning both Scaling-Inputs and Scaling Input-Free Tasks schemes, reveal that LLMs, at various scales, trained on MUFFIN generally demonstrate superior instruction-following capabilities compared to those trained on the two aforementioned schemes.

==> sections/9Acknowledgment.tex <==
We sincerely thank all the reviewers' constructive comments on improving this work.

==> tables/main_table_t5_11b.tex <==

\begin{table*}[ht!]
 \setlength{\belowcaptionskip}{-3pt}
 \setlength{\abovecaptionskip}{6pt}
\centering
% \normalise
\small
\caption{Results on T5-11B. The best scores under direct and indirect comparison settings are in \textbf{bold} and {\ul underlined}, respectively.}
\resizebox{0.98\linewidth}{!}{

\begin{tabular}{lcccc|cc|cc|cc}

\toprule

                                        &                                      & \multicolumn{3}{c}{\textbf{\colorbox{TagBlue}{SuperNI-Test}}}                                                                                                                                                                                                & \multicolumn{2}{c}{\textbf{\colorbox{TagOrange}{MMLU}}}                           & \multicolumn{2}{c}{\textbf{\colorbox{TagGray}{T0-Eval}}}                        & \textbf{\colorbox{TagGray}{BBH}}                 &                                    \\
                                        
                                        \cmidrule{3-10}
                                        
\multirow{-2}{*}{\textbf{Models}}       & \multirow{-2}{*}{\textbf{Data Size}} & \textit{\textbf{\begin{tabular}[c]{@{}c@{}}EM \\ (CLS)\end{tabular}}} & \textit{\textbf{\begin{tabular}[c]{@{}c@{}}ROUGE-L \\ (GEN)\end{tabular}}} & \textit{\textbf{\begin{tabular}[c]{@{}c@{}}ROUGE-L \\ (overall)\end{tabular}}} & \textit{\textbf{Rank ACC}}   & \textit{\textbf{EM}}         & \textit{\textbf{Rank ACC}}   & \textit{\textbf{EM}}         & \textit{\textbf{EM}}         & \multirow{-2}{*}{\textbf{Average}} \\ \midrule
% \multicolumn{11}{c}{\cellcolor[HTML]{C0C0C0}\textit{Larger Models / Vanilla Models / More Training Data (for reference)}}                                                                                                                                                                                                                                                                                                                                                                                            \\
% {\color[HTML]{656565} GPT-4}            & {\color[HTML]{656565} /}             & {\color[HTML]{656565} 64.51}                                          & {\color[HTML]{656565} 59.36}                                               & {\color[HTML]{656565} 62.96}                                                   & {\color[HTML]{656565} /}     & {\color[HTML]{656565} 82.40}\textsuperscript{\rm $\dagger$} & {\color[HTML]{656565} /}     & {\color[HTML]{656565} 70.95} & {\color[HTML]{656565} 67.40}\textsuperscript{\rm *} & {\color[HTML]{656565} /}           \\
% {\color[HTML]{656565} ChatGPT}          & {\color[HTML]{656565} /}             & {\color[HTML]{656565} 46.90}                                          & {\color[HTML]{656565} 56.82}                                               & {\color[HTML]{656565} 52.41}                                                   & {\color[HTML]{656565} /}     & {\color[HTML]{656565} 67.90}\textsuperscript{\rm $\dagger$} & {\color[HTML]{656565} /}     & {\color[HTML]{656565} 50.73} & {\color[HTML]{656565} 48.90}\textsuperscript{\rm *} & {\color[HTML]{656565} /}           \\
% {\color[HTML]{656565} Flan-T5 (11B)}    & {\color[HTML]{656565} 14M}           & {\color[HTML]{656565} NHO}                                            & {\color[HTML]{656565} NHO}                                                 & {\color[HTML]{656565} NHO}                                                     & {\color[HTML]{656565} 49.97} & {\color[HTML]{656565} 45.97} & {\color[HTML]{656565} NHO}   & {\color[HTML]{656565} NHO}   & {\color[HTML]{656565} 40.92} & {\color[HTML]{656565} /}           \\
% {\color[HTML]{656565} Flan-T5 (3B)}     & {\color[HTML]{656565} 14M}           & {\color[HTML]{656565} NHO}                                            & {\color[HTML]{656565} NHO}                                                 & {\color[HTML]{656565} NHO}                                                     & {\color[HTML]{656565} 45.52} & {\color[HTML]{656565} 45.07} & {\color[HTML]{656565} NHO}   & {\color[HTML]{656565} NHO}   & {\color[HTML]{656565} 39.70} & {\color[HTML]{656565} /}           \\
% {\color[HTML]{656565} T0++ (11B)}       & {\color[HTML]{656565} 12M}           & {\color[HTML]{656565} 29.40}                                          & {\color[HTML]{656565} 48.46}                                               & {\color[HTML]{656565} 40.01}                                                   & {\color[HTML]{656565} 45.46} & {\color[HTML]{656565} 43.20} & {\color[HTML]{656565} 59.70} & {\color[HTML]{656565} 62.22} & {\color[HTML]{656565} 20.15} & {\color[HTML]{656565} 43.58}       \\
% {\color[HTML]{656565} T0 (11B)}         & {\color[HTML]{656565} 50K}           & {\color[HTML]{656565} 24.08}                                          & {\color[HTML]{656565} 41.15}                                               & {\color[HTML]{656565} 32.85}                                                   & {\color[HTML]{656565} 42.87} & {\color[HTML]{656565} 40.08} & {\color[HTML]{656565} 57.52} & {\color[HTML]{656565} 60.00} & {\color[HTML]{656565} 29.04} & {\color[HTML]{656565} 40.95}       \\
% {\color[HTML]{656565} T0 (3B)}          & {\color[HTML]{656565} 50K}           & {\color[HTML]{656565} 18.95}                                          & {\color[HTML]{656565} 36.66}                                               & {\color[HTML]{656565} 26.84}                                                   & {\color[HTML]{656565} 31.51} & {\color[HTML]{656565} 25.32} & {\color[HTML]{656565} 46.17} & {\color[HTML]{656565} 46.63} & {\color[HTML]{656565} 22.76} & {\color[HTML]{656565} 31.86}       \\
% {\color[HTML]{656565} Vanilla T5 (11B)} & {\color[HTML]{656565} 0}             & {\color[HTML]{656565} 0.00}                                           & {\color[HTML]{656565} 20.89}                                               & {\color[HTML]{656565} 8.40}                                                    & {\color[HTML]{656565} 22.95} & {\color[HTML]{656565} 0.00}  & {\color[HTML]{656565} 37.56} & {\color[HTML]{656565} 0.00}  & {\color[HTML]{656565} 0.00}  & {\color[HTML]{656565} 11.23}       \\
% {\color[HTML]{656565} Vanilla T5 (3B)}  & {\color[HTML]{656565} 0}             & {\color[HTML]{656565} 0.00}                                           & {\color[HTML]{656565} 21.84}                                               & {\color[HTML]{656565} 10.28}                                                   & {\color[HTML]{656565} 24.12} & {\color[HTML]{656565} 0.00}  & {\color[HTML]{656565} 37.45} & {\color[HTML]{656565} 0.38}  & {\color[HTML]{656565} 0.00}  & {\color[HTML]{656565} 11.76}       \\ \midrule
\multicolumn{11}{c}{\cellcolor[HTML]{C0C0C0}{\color[HTML]{161616} \textit{Human Annotated Data (indirect comparison)}}}                                                                                                                                                                                                                                                                                                                                                                                              \\
\colorbox{TagBlue}{SuperNI}          & 68k & 41.13                & 50.05                & 47.76                & {\ul 54.45}                & {\ul 54.37}                & {\ul 56.89}                & 54.23                & 29.80                & {\ul 48.59}                \\ \midrule
\multicolumn{11}{c}{\cellcolor[HTML]{C0C0C0}\textit{Generated Data   (direct comprison)}}                                                                                                                                                                                                                                                                                                                                                                                                                            \\
% Dolly                                   & 15k                                  & 0.49                                                                  & 34.32                                                                      & 14.52                                                                          & 23.05                        & 0.00                         & 39.84                        & 6.78                         & 5.71                         & 15.59                              \\

\colorbox{TagOrange}{Dolly}            & 15k & 2.71                 & 37.12                & 17.81                & 22.99                & 0.06                 & 49.17                & 23.96                & 10.18                & 20.50                \\
\colorbox{TagOrange}{LongForm}         & 23k & 1.88                 & 38.05                & 16.27                & 23.23                & 0.00                 & 39.85                & 2.79                 & 5.53                 & 15.95                \\
\colorbox{TagOrange}{Alpaca}           & 52k & 25.36                & 47.74          & 39.62                & 30.17                & 8.10                 & 54.48          & 34.90                & 9.28                 & 30.21                \\
\colorbox{TagOrange}{Alpaca-GPT4}      & 52k & 13.65                & 43.19                & 31.46                & 25.58                & 0.00                 & 49.94                & 34.79                & 7.94                 & 25.82                \\
\colorbox{TagOrange}{WizardLM}         & 68k & 4.81                 & 40.43                & 21.26                & 24.63                & 0.01                 & 45.10                & 6.44                 & 4.79                 & 18.43                \\
\colorbox{TagOrange}{Self-Inst.}       & 82k & 28.88                & 44.88                & 36.53                & 28.22                &  32.45          & 48.61                & 41.46                & \textbf{{\ul 31.39}}       & 36.55          \\
\colorbox{TagBlue}{Unnatural Inst.}  & 68k & 41.11          & 47.46                & 45.54                & 34.38          & 22.39                & 43.40                & 41.91                & 12.84                & 36.13                \\
\colorbox{TagBlue}{Dynosaur}         & 66k & \textbf{{\ul 42.02}}       & 47.53                &  46.42          & 27.60                & 24.96                & 42.85                & 43.39          & 9.22                 & 35.50                \\ \midrule
Muffin (Ours)   & 68k & 40.20                & \textbf{{\ul 50.69}}       & \textbf{{\ul48.32}}       & \textbf{41.95}       & \textbf{41.83}       & \textbf{55.38}       & \textbf{{\ul 57.74}}       & 20.53          & \textbf{44.58}       \\ 

\bottomrule

\end{tabular}

}

\label{tab:main_tab_t5_11b}
% \vskip -1em
\end{table*}




